Causality-Enhanced Behavior Sequence Modeling in LLMs for Personalized Recommendation

Recent advancements in recommender systems have focused on leveraging Large Language Models (LLMs) to improve user preference modeling, yielding promising outcomes. However, current LLM-based approaches struggle to fully leverage user behavior sequences, resulting in suboptimal preference modeling for personalized recommendations. In this study, we propose a novel Counterfactual Fine-Tuning (CFT) method to address this issue by explicitly emphasizing the role of behavior sequences when generating recommendations. Specifically, we employ counterfactual reasoning to identify the causal effects of behavior sequences on model output and introduce a task that directly fits the ground-truth labels based on these effects, achieving the goal of explicit emphasis. Additionally, we develop a token-level weighting mechanism to adjust the emphasis strength for different item tokens, reflecting the diminishing influence of behavior sequences from earlier to later tokens during predicting an item. Extensive experiments on real-world datasets demonstrate that CFT effectively improves behavior sequence modeling. Our codes are available at https://github.com/itsmeyjt/CFT.

==> backup/1_intro.tex <==
\section{Introduction}
% LLM based recommendation ---> user histroy behavior modeling
In recent years, there has been growing enthusiasm for developing recommender systems based on Large Language Models (LLMs), with the expectation that LLMs' advanced capabilities could bring a new revolution to recommendation fields. However, the core of recommendation lies in 
user preference modeling,
% user behavior modeling—understanding users' past behaviors on items to infer their future preference—
% inferring users' future preferences based on their past behaviors—
which naturally differs from the tasks LLMs were originally designed for. 
To bridge this gap, existing approaches typically involve leveraging historical user behavior sequences to construct instruction data and then fine-tuning the LLM model using the data. 
This process equips the LLM with the ability to model user behavior, enabling it to infer user preferences based on the provided behavior sequences as well as its internalized knowledge.
Till now, numerous efforts have been made in this direction, resulting in significant progress.
% This process equips LLMs with the ability to model user behavior, learning 
%This enables LLMs to incorporate user behavior modeling, allowing them to infer preferences by learning from the input behavior sequences and leveraging their internalized knowledge.




% To enable LLM to learn recommendations, existing works xxx.
% 现有工作通常将用户历史交互喂到prompt中，然后通过instruction tuning的形式教会LLM学会基于用户行为序列来学会推荐，并期望在这个过程可以激发LLM的world knowledge&reasoning能力来增强Behavior modeling，实现更好的推荐。


% problem: Behavior modeling 能力可能不强，现有工作&our pre experiments

% An explanation with causal graph, affecting the learning of modeling user behavior

% This works focus on solving the problem. 需要怎样来实现。


% Despite the progress made, we find that such existing instruction tuning may not sufficiently inspire LLMs to leverage the behavior sequence. There are two pieces of evidence. Firstly, we conduct an experiment to compare recommendations generated by LLM-based recommenders with and without behavior sequences as inputs, surprisingly finding that they show similar distribution in terms of items with different frequencies. This indicates that LLMs may have not leveraged the behavior sequence sufficiently, but somewhat overly relied on their pretraining knowledge for recommendation. Besides, a previous study revealed that when removing some genre of items from training data, the LLMs would still recommend such data. This also indicates the potential existence of pretraining bias, influencing the full leverage of the behavior sequence. 


% Despite the advancements, we argue that current tuning methods may not sufficiently encourage LLMs to utilize behavior sequences effectively. When building recommender models with LLMs, besides behavior sequence, the LLMs' pre-training knowledge is expected to contribute, providing world knowledge to improve recommendations. However, the knowledge is embedded in the model parameters and can be more easily stimulated and utilized during training than behavior sequence, making the effects wrongly sourced to pretraining knowledge. For example, we find that, when moving the historical sequence from the LLMs' inputs, the recommendation generated by LLMs still shows a similar distribution to that with inputting the sequence.
% Existing works lack a mechanism to emphasize the behavior sequence modeling, potentially leading to the non-full utilization of the behavior sequence information. 

Despite recent progress, we argue that current fine-tuning methods may not effectively promote LLMs' full leverage of behavior sequences. When building recommendation models with LLMs, beyond the inputted past behavior sequence, the LLM's pre-training knowledge is also expected to contribute to predictions as shown in Figure~\ref{1}, providing valuable world knowledge for recommendations. 
% However, since the pre-training knowledge is deeply embedded in the model's parameters, it is more easily activated during training than behavior sequence information. 
However, during tuning, the behavior sequence patterns are more complex to capture, while the pre-training knowledge is directly embedded in the model parameters and thus easier to leverage.
As a result, the model may be more prone to blindly attributing effects to pre-training knowledge, leading to insufficient utilization of the behavior sequences. 
The findings in Figure~\ref{xxx} indicate this potential over-reliance on pre-training: when we removed the past behavior sequence from the input, the resulting recommendations displayed a similar item distribution to those generated with the sequence included. 

% We find that a recent study showed that even when certain item genres were excluded from the training data, LLMs continued to recommend those items. We believe this indicates the potential existence of pretraining bias. 

% limit the full utilization of the behavior sequence. Moreover, s

This work focuses on enhancing the behavior modeling for LLM-based recommendations during tuning. 
Using causal Language to describe the working mechanism of LLMs, there are different latent paths from the total input to output that can produce the target prediction, with some sourcing from the behavior sequences while others are not related to the behavior sequences. Only those related to the behavior sequences are the focus of the behavior modeling. Therefore, to enhance behavior sequence modeling, a feasible solution is to first identify the effects of such paths, i.e., the total effect of behavior sequence on the predictions, and then we just need to emphasize the effect during tuning.

With these considerations, we aim to design a new fine-tuning method that emphasizes behavior sequence modeling when adapting LLMs to recommendations. To achieve this, we propose adding a task that directly uses the total effect of behavior sequence on model output to fit the data label. 
To achieve this, we first leverage the counterfactual technique to estimate the target effect, by comparing the normal predictions (i.e., those with inputting behavior sequences) and the counterfactual predictions (i.e., those without input behavior sequences) and leveraging the obtained difference as the result. Then, we fit the data label with the estimated effects. Notably, the new task is added in a multi-task manner. That means, using the normal predictions to fit the data label is still kept, considering that other information is still usable for predictions. 

Taking a further step, we note that each sample’s prediction involves predicting a set of tokens of the target item. However, we find that simply applying our method equally to all tokens may suffer from low learning efficacy. Indeed, given the prefix tokens of prediction, the predicted item becomes near definite.
That means, given the prefix tokens, the following tokens would become relatively fixed, making the difference between them smaller and more easily reduced.  Therefore, instead of equally applying our emphasizing mechanism, we design a weighting mechanism to emphasize more the causal effects of learning on the prefix tokens. This formulates our final fine-tuning method. As its core lies in utilizing counterfactuals to estimate the causal effect, we name our method \textit{Counterfactual Fine-Tuning (CFT)}.       

% Using the graph for analysis, we can find that the predictions can be produced with different paths, the behavior sequence modeling corresponds to the path with the behavior sequence as the source node. To enhance the behavior modeling, we need to identify and then enhance the effects of these paths on the predictions. 

% We first resort to a causal graph in Figure 1 to describe LLM's working mechanism --- the pre-training knowledge (E) and input (I) determine the predictions (Y).  


% Two key findings support this. First, in an experiment comparing recommendations generated by LLM-based systems with and without behavior sequence inputs, we unexpectedly found similar item distributions are generated. 
% Secondly, 

% This guess was sourced from an observation in a previous study --- when certain item genres were excluded from the training data, LLMs continued to recommend those genres of items.

% This is sourced from an observation from a recent study, that is, even when certain item genres were excluded from the training data, LLMs continued to recommend those genres of items. 

% Two key findings support this. First, in an experiment comparing recommendations generated by LLM-based systems with and without behavior sequence inputs, we unexpectedly found similar item distribution patterns across different frequency categories. This suggests that LLMs may not be fully leveraging the behavior sequences, instead overly relying on their pretraining knowledge for recommendations. Additionally, a previous study showed that even when certain item genres were excluded from the training data, LLMs continued to recommend those items. This further highlights the presence of pretraining biases, which may hinder the full utilization of behavior sequences.

% Despite the progress made, we find that the LLM may suffer from insufficient utilization of behavior sequences. There are two sherds of evidence. First, a previous study revealed that when removing some genre of items from training data, the LLMs would still recommend such data, indicating the potential existence of pretraining bias. Moreover, we find that when moving the historical sequence from the LLMs' inputs, the recommendation generated by LLMs still shows a similar distribution to that with inputting the historical behavior sequence, as shown in Figure~\ref{xxx}.  Both findings indicate LLMs may have not leveraged the behavior sequence sufficiently, but somewhat overly rely on their pretraining knowledge for recommendation.

==> backup/1_intro_1009.tex <==
\section{Introduction}
% LLM based recommendation ---> user histroy behavior modeling
In recent years, there has been growing enthusiasm for developing recommender systems based on Large Language Models (LLMs)~\cite{zoranker,llm4trdrec,li2023prompt, agentcf, lcrec,binllm,tallrec,llmrec_survey}, 
with the expectation that LLMs' advanced capabilities could bring a new revolution to recommendation fields. 
% driven by the expectation that LLMs' advanced capabilities could revolutionize the recommendation field~\cite{}.
However, the core of recommendation lies in user preference modeling~\cite{user_modeling},
% user behavior modeling—understanding users' past behaviors on items to infer their future preference—
% inferring users' future preferences based on their past behaviors—
% which naturally differs from the tasks LLMs were originally designed for. 
which inherently differs from the 
language processing
tasks LLMs were originally designed for~\cite{tallrec}. 
% To bridge this gap, existing approaches typically involve leveraging historical user behavior sequences to construct instruction data and then fine-tuning the LLM model using the data. 
% To bridge this gap, current approaches often leverage historical user behavior sequences to create instruction data, which is then used to fine-tune LLMs~\cite{}.
To bridge this gap, current approaches often construct instruction data from historical user behavior sequences and then use it to fine-tune LLMs~\cite{instructrec,binllm,lcrec}.
% To bridge this gap, current approaches often fine-tune LLMs with instruction data constructed on user historical behavior sequences.
This process equips LLMs with the ability to model user behavior, allowing them to infer user preferences based on the provided behavior sequences and their internalized knowledge.
Till now, numerous efforts have been made in this direction, leading to significant progress~\cite{lcrec,recgpt,d3,transrec,bigrec}.
% This process equips LLMs with the ability to model user behavior, learning 
%This enables LLMs to incorporate user behavior modeling, allowing them to infer preferences by learning from the input behavior sequences and leveraging their internalized knowledge.




% To enable LLM to learn recommendations, existing works xxx.
% 现有工作通常将用户历史交互喂到prompt中，然后通过instruction tuning的形式教会LLM学会基于用户行为序列来学会推荐，并期望在这个过程可以激发LLM的world knowledge&reasoning能力来增强Behavior modeling，实现更好的推荐。


% problem: Behavior modeling 能力可能不强，现有工作&our pre experiments

% An explanation with causal graph, affecting the learning of modeling user behavior

% This works focus on solving the problem. 需要怎样来实现。


% Despite the progress made, we find that such existing instruction tuning may not sufficiently inspire LLMs to leverage the behavior sequence. There are two pieces of evidence. Firstly, we conduct an experiment to compare recommendations generated by LLM-based recommenders with and without behavior sequences as inputs, surprisingly finding that they show similar distribution in terms of items with different frequencies. This indicates that LLMs may have not leveraged the behavior sequence sufficiently, but somewhat overly relied on their pretraining knowledge for recommendation. Besides, a previous study revealed that when removing some genre of items from training data, the LLMs would still recommend such data. This also indicates the potential existence of pretraining bias, influencing the full leverage of the behavior sequence. 


% Despite the advancements, we argue that current tuning methods may not sufficiently encourage LLMs to utilize behavior sequences effectively. When building recommender models with LLMs, besides behavior sequence, the LLMs' pre-training knowledge is expected to contribute, providing world knowledge to improve recommendations. However, the knowledge is embedded in the model parameters and can be more easily stimulated and utilized during training than behavior sequence, making the effects wrongly sourced to pretraining knowledge. For example, we find that, when moving the historical sequence from the LLMs' inputs, the recommendation generated by LLMs still shows a similar distribution to that with inputting the sequence.
% Existing works lack a mechanism to emphasize the behavior sequence modeling, potentially leading to the non-full utilization of the behavior sequence information. 

\begin{figure}[t]
\centering
% \subfigure[\textbf{ML-1M Warm}]{\includegraphics[width=1.475in,height=1.15in]{figures/books_cmp_his.png}}
\subfigure[\textbf{ML-1M Warm}]{\includegraphics[width=0.23\textwidth]{figures/books_cmp_his.png}}
% \vspace{-5pt}
% \subfigure[ \textbf{Amazon-book Warm}]{ \includegraphics[width=1.475in,height=1.15in]{figures/games_cmp_his.png}}
\subfigure[ \textbf{Amazon-book Warm}]{ \includegraphics[width=0.23\textwidth]{figures/games_cmp_his.png}}
% \quad
% \vspace{-15pt}
\caption{Recommendation comparison for LLM-based method BIGRec~\cite{bigrec} between with and without inputting historical behavior sequences.}
\label{fig:cmp-his}
% \vspace{-18pt}
\Description{..}
\end{figure}


% Despite the remarkable progress, we argue that current fine-tuning methods may not effectively promote LLMs' full leverage of behavior sequences. 
Despite the remarkable progress, we argue that current fine-tuning methods may not fully harness the potential of LLMs in effectively utilizing behavior sequences. 
When building recommendation models with LLMs, information unrelated to the input behavior sequence—such as pre-training knowledge triggered by the task instruction—can also be utilized for prediction. 
% When using LLMs as recommender models, information unrelated to the input behavior sequence, such as pre-training knowledge triggered by task instructions, can also contribute to predictions. 
% This information is inherently embedded in LLM parameters and is less complex to 
% % activate for 
% use than the behavior sequence.
This information is inherently embedded in the LLM parameters and is simpler to utilize than the complex behavior-related information.
% is less complex to utilize than behavior-related information.
% Consequently, LLMs may tend to over-rely on this information to fit prediction targets, resulting in insufficient utilization of behavior sequences.
Consequently, LLMs may tend to over-rely on this information when fitting prediction targets, resulting in insufficient utilization of behavior sequences.
% One of our findings indicates potential over-reliance: removing the past behavior sequence from the input still resulted in similar recommendation distributions to those generated with the sequence included, as shown in Figure~\ref{}.
One of our findings indicates this potential insufficient utilization: when removing the user behavior sequence from the input, the LLM-based recommender still produced similar recommendation distributions to those generated with the sequence included, as shown in Figure~\ref{fig:cmp-his}.
% Undoubtedly, insufficient utilization of behavior sequences would hinder effective preference modeling, limiting the model's performance.  


% When building recommendation models with LLMs, beyond the inputted past behavior sequence, the LLM's pre-training knowledge is also expected to contribute to predictions as shown in Figure~\ref{1}, providing valuable world knowledge for recommendations. 
% However, since the pre-training knowledge is deeply embedded in the model's parameters, it is more easily activated during training than behavior sequence information. 
% However, the behavior sequence patterns are more complex to capture, while the pre-training knowledge is directly embedded in the model parameters and thus easier to leverage.
% As a result, the model may be more prone to blindly attributing effects to pre-training knowledge, leading to insufficient utilization of the behavior sequences. 
% The findings in Figure~\ref{xxx} indicate this potential over-reliance on pre-training: when we removed the past behavior sequence from the input, the resulting recommendations displayed a similar item distribution to those generated with the sequence included. 

% We find that a recent study showed that even when certain item genres were excluded from the training data, LLMs continued to recommend those items. We believe this indicates the potential existence of pretraining bias. 

% limit the full utilization of the behavior sequence. Moreover, s


% Insufficient utilization of behavior sequences would undoubtedly hinder effective preference modeling, limiting the model's performance. In this work, we focuses on solving the problem. 
% It is essential to enhance behavior sequence modeling in LLM-based recommendation, considering its fundamental role for user preference mining. 
% We resort to causal graph in Figure~\ref{} to analyze the problem. 


Given the central role of behavior modeling in recommendations, it is crucial to address the problem of insufficient utilization of behavior sequences in LLM-based recommendations. To tackle this issue, we first employ \textit{causal language}~\cite{pearl2009causality} for a qualitative analysis. As illustrated in Figure~\ref{fig:causal_graph}, given input features, LLMs can generate predictions through various causal paths, some of which do not originate from the behavior sequence. The insufficient utilization of behavior sequences arises from the tendency to overlook the effects of behavior sequence-originated paths compared to others. Therefore, to enhance behavior sequence modeling, 
the key is to identify the effects of these behavior sequence-originated paths, which correspond to the total causal effect of behavior sequences on predictions, and emphasize these effects during the tuning process. 



% Building on the above finding, we first approach the problem of behavior sequence modeling in LLM-based recommendations from a causal perspective.
% % As the figure shows, 
% As illustrated in Figure~\ref{},
% % given inputs, LLMs can generate predictions through various causal paths, some of which do not originate from the behavior sequence. 
% given input features, LLMs can generate predictions through various causal paths, some of which do not originate from the behavior sequence.
% % The insufficient utilization of behavior sequences stems from the tendency to overlook the effects of the behavior sequence-originated paths, compared to others. 
% The insufficient utilization of behavior sequences arises from the tendency to overlook the effects of behavior-sequence-originated paths compared to others.
% % Therefore, to improve behavior sequence modeling, we think the key is to identify the effects of these behavior sequence-originated paths, which correspond to the total causal effect of behavior sequences on predictions, and to emphasize these effects during tuning.
% Therefore, to enhance behavior sequence modeling, it is crucial to identify the effects of these behavior-sequence-originated paths, which correspond to the total causal effect of behavior sequences on predictions, and to emphasize these effects during the tuning process.

% Using causal Language to describe the working mechanism of LLMs, there are different latent paths from the total input to output that can produce the target prediction, with some sourcing from the behavior sequences while others are not related to the behavior sequences. Only those related to the behavior sequences are the focus of the behavior modeling. Therefore, to enhance behavior sequence modeling, a feasible solution is to first identify the effects of such paths, i.e., the total effect of behavior sequence on the predictions, and then we just need to emphasize the effect during tuning.

% To this end, we propose to emphasize the causal effect of behavior sequence on the predictions to enhance behavior sequence modeling. 

% To this end, we propose a new fine-tuning method that emphasizes the effects of behavior sequences on predictions to enhance behavior sequence modeling in LLMs.
% To this end, we propose a novel fine-tuning method that explicitly highlights the previously neglected effects.

To this end, we propose a novel fine-tuning method, which explicitly emphasizes behavior sequences' effects on LLM predictions during tuning to enhance behavior modeling. Specifically, we leverage counterfactual reasoning~\cite{pearl2009causality,pearl2016primer} to estimate the effects as the difference between normal predictions (i.e., those generated using behavior sequences) and counterfactual predictions (i.e., those generated without them).  
We then introduce a new task that directly uses the estimated effects to fit the ground-truth labels, explicitly attributing the label occurrences to these effects, achieving the intended emphasis.  
This task is integrated into the tuning in a multi-task manner~\cite{multitask}, allowing us to retain the original task of fitting labels with normal predictions, thereby preserving other valuable information relevant to the task.  

% The emphasis is achieved by introducing a new task that directly leverages these effects to fit the ground-truth labels. 
% Specifically, through counterfactual reasoning, we first estimate the effects as the difference between normal predictions (i.e., those obtained using behavior sequences) and counterfactual predictions (i.e., those obtained without the sequences), and then fit labels with the obtained difference.
% % Firstly, we leverage counterfactual reasoning to estimate the effects as the difference between normal predictions (i.e., those obtained using behavior sequences) and counterfactual predictions (i.e., those obtained without the sequences). Subsequently, we utilize the difference to directly fit the labels.
% Notably, this additional task is added in a multi-task framework, allowing us to retain the original task of using normal predictions to fit the labels, thereby preserving other valuable information.






% To this end, we propose a novel fine-tuning method that can enhance behavior sequence modeling by emphasizing the effects of behavior sequences on predictions during tuning.
% We achieve this by adding a new task that directly utilizes the total effect of behavior sequences on model output to fit the data labels. 
% We achieve this by introducing a new task that directly leverages these effects to fit the ground-truth labels.
% Specifically, using counterfactual reasoning, we first estimate the effect as the difference between normal predictions (\ie, those obtained with inputting behavior sequences) and counterfactual predictions (\ie, those obtained without the sequences). We then use this difference to directly fit the data labels. 
% Specifically, through counterfactual reasoning, we first estimate this effect as the difference between normal predictions (i.e., those obtained using behavior sequences) and counterfactual predictions (i.e., those obtained without the sequences), and then utilize this difference to directly fit the labels.
% % Notably, this new task is integrated in a multi-task manner, allowing us to retain the task of using normal predictions to fit data labels, thereby preserving other valuable information.
% Notably, this additional task is integrated in a multi-task framework, allowing us to retain the original task of using normal predictions to fit the labels, thereby preserving other valuable information.

% Notably, the new task is added in a multi-task manner. That means, using the normal predictions to fit the data label is still kept, considering that other information is still usable for predictions. 

% we compare the normal predictions (i.e., those with inputting behavior sequences) and the counterfactual predictions (i.e., those without input behavior sequences)

% The effect is estimated based on counterfactuals --- the normal predictions (i.e., those with inputting behavior sequences) and the counterfactual predictions (i.e., those without input behavior sequences).

% With these considerations, we aim to design a new fine-tuning method that emphasizes behavior sequence modeling when adapting LLMs to recommendations. To achieve this, we propose adding a task that directly uses the total effect of behavior sequence on model output to fit the data label. 
% To achieve this, we first leverage the counterfactual technique to estimate the target effect, by comparing the normal predictions (i.e., those with inputting behavior sequences) and the counterfactual predictions (i.e., those without input behavior sequences) and leveraging the obtained difference as the result. Then, we fit the data label with the estimated effects. Notably, the new task is added in a multi-task manner. That means, using the normal predictions to fit the data label is still kept, considering that other information is still usable for predictions. 

% Taking a further step, for recommendation, each sample’s prediction involves predicting a set of tokens of the target item, however, simply applying our method equally to all tokens may suffer from overfitting to the later tokens. 
% Specifically, once more prefix tokens are established, the predicted item becomes more definite. That means, for subsequent tokens, the uncertainty would become smaller, and thus the differences between normal and counterfactual predictions would naturally be smaller and easier to diminish than the prefix ones. Equally treating all tokens would undoubtedly lead to our tuning focus on these less important later tokens, preventing its actual effects.  
% To overcome the issue, we additionally design a mechanism to adaptively assign higher weights to prefix during applying emphasizing the causal effects. This formulates our final fine-tuning method. As its core lies in utilizing counterfactuals to estimate the causal effect, we name our method \textit{Counterfactual Fine-Tuning (CFT)}. 
% Taking a further step, we observe that in recommendation tasks, each sample's prediction involves predicting a sequence of tokens for the target item. However, simply applying our method equally to all tokens may limit its effectiveness. Specifically, for item prediction, as more prefix tokens are established, the prediction becomes more definite. In other words, the uncertainty in predicting the later tokens decreases. That means that for these tokens, the difference between normal predictions and counterfactual predictions, i.e., the causal effect of the behavior sequence, naturally becomes smaller. At this point, forcing the causal effect that gradually approaches 0 to fit the target becomes inappropriate. To address this issue, we introduce a mechanism that adaptively assigns higher weights to the former tokens when emphasizing the causal effects on predictions. This forms our final fine-tuning method. Since the method centers on utilizing counterfactuals to estimate and emphasize causal effects, we name it Counterfactual Fine-Tuning (CFT).
Taking a further step, we observe that in the recommendation task, each sample's prediction usually involves forecasting a sequence of tokens corresponding to the next item.
% However, applying our method uniformly across all tokens may limit its effectiveness. 
However, uniformly applying our method to all tokens may hinder its effectiveness. Specifically, as more prefix tokens are established, the prediction for an item becomes increasingly certain, leading to reduced uncertainty in predicting subsequent tokens.
Consequently, the difference between normal and counterfactual predictions—\textit{i.e.,} the causal effect of the behavior sequence—naturally diminishes on these later tokens. In other words, the prediction of these tokens is increasingly less influenced by the behavior sequence.
In this case, uniformly forcing these diminishing causal effects (even approaching zero) to fit data labels becomes inappropriate.
To tackle the challenge, we introduce a mechanism that adaptively assigns greater weights to earlier tokens when emphasizing the causal effects on predictions, forming our final fine-tuning method. Since the method centers on using counterfactuals to estimate and emphasize causal effects, we name it Counterfactual Fine-Tuning (CFT).

The main contributions of this work are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We highlight the issue of insufficient utilization of behavior sequences in existing LLM-based recommendation methods and provide an analysis from a causal perspective.
    
    % \item We propose a new counterfactual fine-tuning method to enhance behavior modeling in LLM-based recommendations by focusing on learning the effects of behavior sequences on predictions. To our knowledge, this is the first approach to integrate causality into LLM-based recommendations.
    
    \item We propose a novel counterfactual fine-tuning method to enhance behavior modeling in LLM-based recommendations by explicitly emphasizing the effects of behavior sequences on predictions during tuning. 
    %To our knowledge, this is the first approach to incorporate causality into LLM tuning for recommendation systems.
    
    \item We conduct extensive experiments on several real-world datasets, demonstrating the effectiveness of our method in enhancing behavior sequence modeling.
\end{itemize}



% That means, given the prefix tokens, the following tokens would become relatively fixed, making the difference between them smaller and more easily reduced.  Therefore, instead of equally applying our emphasizing mechanism, we design a weighting mechanism to emphasize more the causal effects of learning on the prefix tokens. This formulates our final fine-tuning method. As its core lies in utilizing counterfactuals to estimate the causal effect, we name our method \textit{Counterfactual Fine-Tuning (CFT)}.       

% Using the graph for analysis, we can find that the predictions can be produced with different paths, the behavior sequence modeling corresponds to the path with the behavior sequence as the source node. To enhance the behavior modeling, we need to identify and then enhance the effects of these paths on the predictions. 

% We first resort to a causal graph in Figure 1 to describe LLM's working mechanism --- the pre-training knowledge (E) and input (I) determine the predictions (Y).  


% Two key findings support this. First, in an experiment comparing recommendations generated by LLM-based systems with and without behavior sequence inputs, we unexpectedly found similar item distributions are generated. 
% Secondly, 

% This guess was sourced from an observation in a previous study --- when certain item genres were excluded from the training data, LLMs continued to recommend those genres of items.

% This is sourced from an observation from a recent study, that is, even when certain item genres were excluded from the training data, LLMs continued to recommend those genres of items. 

% Two key findings support this. First, in an experiment comparing recommendations generated by LLM-based systems with and without behavior sequence inputs, we unexpectedly found similar item distribution patterns across different frequency categories. This suggests that LLMs may not be fully leveraging the behavior sequences, instead overly relying on their pretraining knowledge for recommendations. Additionally, a previous study showed that even when certain item genres were excluded from the training data, LLMs continued to recommend those items. This further highlights the presence of pretraining biases, which may hinder the full utilization of behavior sequences.

% Despite the progress made, we find that the LLM may suffer from insufficient utilization of behavior sequences. There are two sherds of evidence. First, a previous study revealed that when removing some genre of items from training data, the LLMs would still recommend such data, indicating the potential existence of pretraining bias. Moreover, we find that when moving the historical sequence from the LLMs' inputs, the recommendation generated by LLMs still shows a similar distribution to that with inputting the historical behavior sequence, as shown in Figure~\ref{xxx}.  Both findings indicate LLMs may have not leveraged the behavior sequence sufficiently, but somewhat overly rely on their pretraining knowledge for recommendation.

==> backup/1_intro_compare_1008.tex <==
%原版VS修改

%P1
In recent years, there has been growing enthusiasm for developing recommender systems based on Large Language Models (LLMs), with the expectation that LLMs' advanced capabilities could bring a new revolution to recommendation fields. However, the core of recommendation lies in user preference modeling, which naturally differs from the tasks LLMs were originally designed for. To bridge this gap, existing approaches typically involve leveraging historical user behavior sequences to construct instruction data and then fine-tuning the LLM model using the data. This process equips LLMs with the ability to model user behavior, enabling them to infer user preferences based on the provided behavior sequences as well as their internalized knowledge. Till now, numerous efforts have been made in this direction, leading to significant progress.

In recent years, there has been growing enthusiasm for developing recommender systems based on Large Language Models (LLMs), driven by the expectation that LLMs' advanced capabilities could revolutionize the recommendation field~\cite{}. However, the core of recommendation lies in user preference modeling, which inherently differs from the language processing tasks LLMs were originally designed for~\cite{}. To bridge this gap, current approaches often leverage historical user behavior sequences to create instruction data, which is then used to fine-tune LLMs~\cite{}. This process equips LLMs with the ability to model user behavior, allowing them to infer user preferences based on the provided behavior sequences as well as their internalized knowledge. Till now, numerous efforts have been made in this direction, leading to significant progress~\cite{}.

%P2
Despite the remarkable progress, we argue that current fine-tuning methods may not effectively promote LLMs' full leverage of behavior sequences. When building recommendation models with LLMs, information unrelated to the input behavior sequence—such as pre-training knowledge triggered by the task instruction—can also be utilized for prediction. This information is inherently embedded in LLM parameters and is less complex to use than the behavior sequence. Consequently, LLMs may tend to over-rely on this information to fit prediction targets, resulting in insufficient utilization of behavior sequences. One of our findings indicates potential over-reliance: removing the past behavior sequence from the input still resulted in similar recommendation distributions to those generated with the sequence included, as shown in Figure~\ref{}.

Despite the remarkable progress, we argue that current fine-tuning methods may not fully harness the potential of LLMs in effectively utilizing behavior sequences. When using LLMs as recommender models, information unrelated to the input behavior sequence, such as pre-training knowledge triggered by task instructions, can also contribute to predictions. This information is inherently embedded in LLM parameters and is less complex to employ than behavioral data. Consequently, LLMs may tend to over-rely on this information when fitting prediction targets, resulting in insufficient utilization of behavior sequences. One of our findings indicates this potential over-reliance: removing the past behavior sequence from the input still produced similar recommendation distributions to those generated with the sequence included, as shown in Figure~\ref{}.

%P3
It is essential to enhance behavior sequence modeling in LLM-based recommendation, considering its fundamental role for user preference mining. We resort to causal graph in Figure~\ref{} to analyze the problem. As the figure shows, given inputs, LLMs can generate predictions through various causal paths, some of which do not originate from the behavior sequence. The insufficient utilization of behavior sequences stems from the tendency to overlook the effects of the behavior sequence-originated paths, compared to others. Therefore, to improve behavior sequence modeling, we think the key is to identify the effects of these behavior sequence-originated paths, which correspond to the total causal effect of behavior sequences on predictions, and to emphasize these effects during tuning.

Building on the above finding, we first approach the problem of behavior sequence modeling in LLM-based recommendations from a causal perspective. As illustrated in Figure~\ref{}, given input features, LLMs can generate predictions through various causal paths, some of which do not originate from the behavior sequence. The insufficient utilization of behavior sequences arises from the tendency to overlook the effects of behavior-sequence-originated paths compared to others. Therefore, to enhance behavior sequence modeling, it is crucial to identify the effects of these behavior-sequence-originated paths, which correspond to the total causal effect of behavior sequences on predictions, and to emphasize these effects during the tuning process.

%P4
To this end, we propose a new fine-tuning method that emphasizes the effects of behavior sequences on predictions to enhance behavior sequence modeling in LLMs. We achieve this by adding a new task that directly utilizes the total effect of behavior sequences on model output to fit the data labels. Specifically, using counterfactual reasoning, we first estimate the effect as the difference between normal predictions (\ie, those obtained with inputting behavior sequences) and counterfactual predictions (\ie, those obtained without the sequences). We then use this difference to directly fit the data labels. Notably, this new task is integrated in a multi-task manner, allowing us to retain the task of using normal predictions to fit data labels, thereby preserving other valuable information.

To this end, we propose a novel fine-tuning method that explicitly highlights the previously neglected effects. We achieve this by introducing a new task that directly leverages the total effect of behavior sequences on the model predictions to align with the ground-truth labels. Specifically, through counterfactual reasoning, we first estimate this effect as the difference between normal predictions (i.e., those obtained using behavior sequences) and counterfactual predictions (i.e., those obtained without the sequences), and then utilize this difference to directly fit the labels. Notably, this additional task is integrated in a multi-task framework, allowing us to retain the original task of using normal predictions to fit the labels, thereby preserving other valuable information.

%P5
Taking a further step, we observe that in recommendation tasks, each sample's prediction involves predicting a sequence of tokens for the target item. However, simply applying our method equally to all tokens may limit its effectiveness. Specifically, for item prediction, as more prefix tokens are established, the prediction becomes more definite. In other words, the uncertainty in predicting the later tokens decreases. That means that for these tokens, the difference between normal predictions and counterfactual predictions, i.e., the causal effect of the behavior sequence, naturally becomes smaller. At this point, forcing the causal effect that gradually approaches 0 to fit the target becomes inappropriate. To address this issue, we introduce a mechanism that adaptively assigns higher weights to the former tokens when emphasizing the causal effects on predictions. This forms our final fine-tuning method. Since the method centers on utilizing counterfactuals to estimate and emphasize causal effects, we name it Counterfactual Fine-Tuning (CFT).

Taking a further step, we observe that in recommendation tasks, each sample's prediction requires generating a sequence of tokens corresponding to the target item. However, applying our method uniformly across all tokens may limit its effectiveness. Specifically, for item prediction, as more prefix tokens are established, the prediction becomes more definite, reducing the uncertainty for predicting subsequent tokens. Consequently, the difference between normal predictions and counterfactual predictions, i.e., the causal effect of the behavior sequence, naturally diminishes for these tokens. At this stage, forcing a diminishing causal effect to fit the target prediction becomes impractical.
To tackle this challenge, we further introduce a mechanism that adaptively assigns greater weights to earlier tokens when emphasizing the causal effects on predictions, which forms our ultimate fine-tuning method. Since the method revolves around the utilization of counterfactuals to estimate and emphasize causal effects, we refer to it as Counterfactual Fine-Tuning (CFT).

%P6
The main contributions of this work are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We highlight the issue of insufficient utilization of behavior sequences in existing LLM-based recommendation methods and provide an analysis from a causal perspective.
    
    \item We propose a new counterfactual fine-tuning method to enhance behavior modeling in LLM-based recommendations by focusing on learning the effects of behavior sequences on predictions. To our knowledge, this is the first approach to integrate causality into LLM-based recommendations.

    \item We conduct extensive experiments on several real-world datasets, demonstrating the effectiveness of our method in enhancing behavior modeling.
\end{itemize}

The main contributions of this work are summarized as follows:
\begin{itemize}[leftmargin=*]
    \item We highlight the issue of insufficient utilization of behavior sequences in existing LLM-based recommendation methods and provide an analysis from a causal perspective.
    
    \item We propose a novel counterfactual fine-tuning method to enhance behavior modeling in LLM-based recommendations by explicitly highlighting the effects of behavior sequences on predictions. To the best of our knowledge, this is the first approach to integrate causality into LLM-based recommendations.
    
    \item We conduct extensive experiments on several real-world datasets, demonstrating the effectiveness of our method in enhancing behavior sequence modeling.
\end{itemize}

==> backup/4_exp.tex <==
% Please add the following required packages to your document preamble:
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\section{Experiment}
In this section, we conduct a series of experiments to answer the
following research questions:

\noindent \textbf{RQ1}: How does CFT perform on real-world datasets compared to existing sequential recommendation methods?

\noindent \textbf{RQ2}: What is the impact of the individual components of CFT on its effectiveness?

\noindent \textbf{RQ3}: How do the specific hyper-parameters of CFT influence its recommendation performance?

\subsection{Experimental Settings}
\subsubsection{Datasets}
% We conduct extensive experiments on three datasets from Amazon Review Data, including \textit{CDs}, \textit{Games}, and \textit{Books}. All datasets contain user review data between 1996 and 2018. 
We conduct extensive experiments on datasets from Amazon Review Data~\cite{amazon}, which contains 233.1 million reviews from May 1996 to October 2018. In particular, we select categories of CDs, Games, and Books for subsequent evaluation. The summary statistics of the three datasets are presented in Table~\ref{table:dataset}.

\begin{table}[t]
\caption{Statistical details of the evaluation datasets.}
\label{table:dataset}
\begin{tabular}{cccc}
\hline
Dataset & \#user & \#item & \#interaction \\ \hline
CDs     & 21,347       &  14,239      &   185,855            \\
Games   & 34,089       &  11,037      &   252,015            \\
Books   &  67,708      &  41,722       &    853,747           \\ \hline
\end{tabular}
\end{table}

% For data preprocessing, we first filter out unpopular users and items with fewer than five interactions, and set the maximum number of item sequence to 10. Then, the data is sorted in chronological order and divided into training, validation, and test sets with a ratio of 8:1:1.
For data preprocessing, we implement a 5-core filtering process to ensure that each user and video has a minimum of 5 samples. Subsequently, we split the data into training, validation, and test sets based on the timestamps of the interactions, following an 8:1:1 ratio. This chronological partitioning ensures that the predicted interactions during testing occur after all interactions observed during training, thereby preventing information leakage.
For the behavior sequence, we first pad user interaction histories shorter than 11 interactions to a fixed length of 11. We then apply a sliding window of length 11 to extract sequences. In each sequence, the last item serves as the prediction target, while the preceding items form the historical interaction sequence.

\subsubsection{Evaluation Metrics}
% We employ two commonly used metrics to evaluate the model's top-k recommendation performance(accuracy): Hit Ratio (HR@K) and Normalized Discounted Cumulative Gain (NDCG@K), which we compute using the all-ranking protocol. In this paper, we set K as 5 and 10. 
Following prior research~\cite{bigrec,sasrec}, we define the input historical interaction sequence for each testing interaction as the set of interactions that occurred immediately before it. To conduct a comprehensive evaluation of recommendation performance, we utilize two widely recognized accuracy metrics: Hit Ratio (HR@$k$) and Normalized Discounted Cumulative Gain (NDCG@$k$), with $k\in\{5,10\}$. We compute these metrics using the all-ranking protocol~\cite{dros}, where all items that a user has not interacted with are considered potential candidates.

\subsubsection{Baselines}
% We adopt the following sequential
% recommendation models as baselines for our experimental comparison:\\
% $\bullet$ \textbf{Caser:} This is a model that leverages convolutional neural networks (CNNs) to analyze user-item interactions and generate personalized recommendations.\\
% $\bullet$ \textbf{GRU4Rec:} This is an RNN-based
% method that uses Gated Recurrent Units (GRU) to model the user behavior
% via encoding the item sequence. \\
% $\bullet$ \textbf{SASRec:} This is a representative recommendation method using Transformer to model the item sequences.\\
% $\bullet$ \textbf{BIGRec:} This is a method that uses
% instruction-tuning to directly generate items. We
% have made changes to the grounding method of
% this approach. Moreover, we perform the decoding method by set the length penalty to 0 to remove the amplification bias.  

We compare our method against both traditional and LLM-based sequential recommendation methods.
\begin{itemize}[leftmargin=*]
    \item \textbf{Caser}~\cite{caser}. This method utilizes CNN to encode historical interaction sequences.
    \item \textbf{GRU4Rec}~\cite{gru4rec}. This is an RNN-based approach uses Gated Recurrent Units (GRU) to encode historical interactions.
    \item \textbf{SASRec}~\cite{sasrec}. This is a representative transformer-based sequential recommendation approach.
    \item \textbf{BIGRec}~\cite{bigrec}. This method follows a bi-step grounding paradigm, first fine-tuning LLMs to generate meaningful tokens, and then identifying the corresponding actual items.
    \item $\bm{D^3}$~\cite{d3}. This decoding method addresses the amplification bias in LLM-based recommendations by removing length normalization and incorporating a text-free model to assist in decoding. Specifically, we employ the version that applies it to BIGRec.
\end{itemize}

For fair comparisons, we instantiate our proposed CFT based on the two aforementioned LLM-based methods, referred to as \textbf{BIGRec+CFT} and $\bm{D^3}$\textbf{+CFT}, respectively.

% $\bullet$ \textbf{Caser:} This is a model that leverages convolutional neural networks (CNNs) to analyze user-item interactions and generate personalized recommendations.\\
% $\bullet$ \textbf{GRU4Rec:} This is an RNN-based
% method that uses Gated Recurrent Units (GRU) to model the user behavior
% via encoding the item sequence. \\
% $\bullet$ \textbf{SASRec:} This is a representative recommendation method using Transformer to model the item sequences.\\
% $\bullet$ \textbf{BIGRec:} This is a method that uses
% instruction-tuning to directly generate items. We
% have made changes to the grounding method of
% this approach. Moreover, we perform the decoding method by set the length penalty to 0 to remove the amplification bias.  



\subsubsection{Implementing Details} We implement all the experiments using PyTorch 2.0. We use the AdamW optimizer for all the methods. For LLM-based methods, we apply
Qwen2-0.5B as the backbone
LLM and employ Cross-Entropy as the optimization loss. We set the learning rate to 1e-4 and the dropout to 0.05. Different From the original grounding method of BIGRec, we set the number of beam search candidates to 5 and select a total of 10 real items, consisting of the nearest and second-nearest neighbors of the 5 generated items. These items are arranged in the order of the first 5 being the nearest neighbors and the latter 5 being the second-nearest neighbors. The order of the 5 nearest items is consistent with the order generated by beam search, and the same applies to the second-nearest items. For the traditional recommendation models, we optimize them using binary cross-entropy loss(BCE). For hyperparameters, we explore the learning rate
within the range of [1e-2, 1e-3, 1e-4] and adjust the weight decay
within the range of [1e-2, 1e-3, 1e-4, 1e-5, 1e-6].


% \subsection{Main Results}
% In this subsection, we employ our method on three datasets and compare the results with all baselines. As shown in Table 1, it presents our main experimental results. From the table, we have the following observations: \\
% \begin{table*}[t]
% \centering
% \caption{Recommendation accuracy of the compared methods on three datasets.“$\textbf{CFT}$” denotes applying our method to  BIGRec by adjusting two parameters . “$D^3$” denotes removing the amplification bias from BIGRec's decoding. The best results are bolded.}
% \begin{tabular}{clccccccc}
% \hline
% {\color[HTML]{333333} Dataset}                                                                                & \multicolumn{1}{c}{{\color[HTML]{333333} Metrics}} & {\color[HTML]{333333} Caser}  & {\color[HTML]{333333} GRU4Rec} & {\color[HTML]{333333} SASRec} & {\color[HTML]{333333} BIGRec} & {\color[HTML]{333333} $D^3$} & {\color[HTML]{333333} \textbf{BIGRec+CFT}} & {\color[HTML]{333333} \textbf{$D^3$+CFT}} \\ \hline
% {\color[HTML]{333333} }                                                                                       & {\color[HTML]{333333} NDCG@5}                      & {\color[HTML]{333333} 0.0161} & {\color[HTML]{333333} 0.0248}  & {\color[HTML]{333333} 0.0477} & {\color[HTML]{333333} 0.0780}              & {\color[HTML]{333333} 0.0906}                               & {\color[HTML]{333333} 0.0855}               & {\color[HTML]{333333} \textbf{0.0972}}                       \\
% {\color[HTML]{333333} }                                                                                       & {\color[HTML]{333333} HR@5}                        & {\color[HTML]{333333} 0.0224} & {\color[HTML]{333333} 0.0342}  & {\color[HTML]{333333} 0.0647} & {\color[HTML]{333333} 0.1131}              & {\color[HTML]{333333} 0.1243}                               & {\color[HTML]{333333} 0.1309}               & {\color[HTML]{333333} \textbf{0.1417}}                       \\
% {\color[HTML]{333333} }                                                                                       & {\color[HTML]{333333} NDCG@10}                     & {\color[HTML]{333333} 0.0193} & {\color[HTML]{333333} 0.0288}  & {\color[HTML]{333333} 0.0535} & {\color[HTML]{333333} 0.0945}              & {\color[HTML]{333333} 0.1103}                               & {\color[HTML]{333333} 0.1056}               & {\color[HTML]{333333} \textbf{0.1203}}                       \\
% \multirow{-4}{*}{{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}CDs\\ $\alpha$=0.025\\ $\beta$=$\frac{1}{26}$\end{tabular}}}  & {\color[HTML]{333333} HR@10}                       & {\color[HTML]{333333} 0.0485} & {\color[HTML]{333333} 0.0467}  & {\color[HTML]{333333} 0.0824} & {\color[HTML]{333333} 0.1631}              & {\color[HTML]{333333} 0.1826}                               & {\color[HTML]{333333} 0.1925}               & {\color[HTML]{333333} \textbf{0.2116}}                       \\ \hline
% {\color[HTML]{333333} }                                                                                       & {\color[HTML]{333333} NDCG@5}                      & {\color[HTML]{333333} 0.0122} & {\color[HTML]{333333} 0.0169}  & {\color[HTML]{333333} 0.0237} & {\color[HTML]{333333} 0.0377}              & {\color[HTML]{333333} 0.0432}                               & {\color[HTML]{333333} 0.0398}               & {\color[HTML]{333333} \textbf{0.0453}}                       \\
% {\color[HTML]{333333} }                                                                                       & {\color[HTML]{333333} HR@5}                        & {\color[HTML]{333333} 0.0187} & {\color[HTML]{333333} 0.0261}  & {\color[HTML]{333333} 0.0338} & {\color[HTML]{333333} 0.0565}              & {\color[HTML]{333333} 0.0631}                               & {\color[HTML]{333333} 0.0608}               & {\color[HTML]{333333} \textbf{0.0674}}                       \\
% {\color[HTML]{333333} }                                                                                       & {\color[HTML]{333333} NDCG@10}                     & {\color[HTML]{333333} 0.0164} & {\color[HTML]{333333} 0.0221}  & {\color[HTML]{333333} 0.0290} & {\color[HTML]{333333} 0.0434}              & {\color[HTML]{333333} 0.0498}                               & {\color[HTML]{333333} 0.0451}               & {\color[HTML]{333333} \textbf{0.0516}}                       \\
% \multirow{-4}{*}{{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}Games\\ $\alpha$=0.02\\ $\beta$=$\frac{1}{3} $\end{tabular}}}  & {\color[HTML]{333333} HR@10}                       & {\color[HTML]{333333} 0.0321} & {\color[HTML]{333333} 0.0423}  & {\color[HTML]{333333} 0.0502} & {\color[HTML]{333333} 0.0742}              & {\color[HTML]{333333} 0.0836}                               & {\color[HTML]{333333} 0.0775}               & {\color[HTML]{333333} \textbf{0.0868}}                       \\ \hline
% {\color[HTML]{333333} }                                                                                       & {\color[HTML]{333333} NDCG@5}                      & {\color[HTML]{333333} 0.0042} & {\color[HTML]{333333} 0.0060}  & {\color[HTML]{333333} 0.0097} & {\color[HTML]{333333} 0.0260}              & {\color[HTML]{333333} 0.0261}                               & {\color[HTML]{333333} 0.0292}               & {\color[HTML]{333333} \textbf{0.0298}}                       \\
% {\color[HTML]{333333} }                                                                                       & {\color[HTML]{333333} HR@5}                        & {\color[HTML]{333333} 0.0069} & {\color[HTML]{333333} 0.0094}  & {\color[HTML]{333333} 0.0146} & {\color[HTML]{333333} 0.0394}              & {\color[HTML]{333333} 0.0375}                               & {\color[HTML]{333333} \textbf{0.0449}}      & {\color[HTML]{333333} 0.0435}                                \\
% {\color[HTML]{333333} }                                                                                       & {\color[HTML]{333333} NDCG@10}                     & {\color[HTML]{333333} 0.0060} & {\color[HTML]{333333} 0.0078}  & {\color[HTML]{333333} 0.0123} & {\color[HTML]{333333} 0.0333}              & {\color[HTML]{333333} 0.0329}                               & {\color[HTML]{333333} 0.0359}               & {\color[HTML]{333333} \textbf{0.0363}}                       \\
% \multirow{-4}{*}{{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}Books\\ $\alpha$=0.1\\ $\beta$=$\frac{1}{1.2}$\end{tabular}}} & {\color[HTML]{333333} HR@10}                       & {\color[HTML]{333333} 0.0123} & {\color[HTML]{333333} 0.0149}  & {\color[HTML]{333333} 0.0226} & {\color[HTML]{333333} 0.0612}              & {\color[HTML]{333333} 0.0585}                               & {\color[HTML]{333333} \textbf{0.0655}}      & {\color[HTML]{333333} 0.0635}                                \\ \hline
% \end{tabular}
% \end{table*}

% $\bullet$ Compared to the baselines, our approach outperforms them in all metrics on all datasets. The outcomes shows the excellence of our method in  recommendation. \\
% $\bullet$ The decoding method may not be applicable to all datasets. The recommendation performance of the two datasets, \textit{CDs} and \textit{Games}, improves after employing the decoding method. However, after applying this decoding method on the \textit{Books} dataset, there was a slight decrease in the metrics HR@5 and HR@10 compared to the scenario without its use. Additionally, the improvements observed in the metrics NDCG@5 and NDCG@10 were minimal.\\
% $\bullet$ It can be observed that the parameters (\bm{$\alpha$} and \bm{$\beta$}) used for different datasets vary, as our experiments revealed that the suitable parameter ranges differ across datasets. More details are mentioned in \ref{4.3.1}. 

\subsection{Performance Comparison (RQ1)}
\begin{table*}[t]

\caption{Performance comparison between the baselines and our proposed CFT on three datasets with NDCG@$k$ (NG@$k$) and HR@$k$ as the metrics. The best results are
highlighted in bold and sub-optimal results are underlined. }
\label{exp:main}

\resizebox{0.98\textwidth}{!}{
\begin{tabular}{ccccccccccccccc}
\cline{1-10} \cline{12-15}
\multirow{2}{*}{Method} & \multicolumn{4}{c}{CDs}                                               &           & \multicolumn{4}{c}{Games}                                             &  & \multicolumn{4}{c}{Books}                                             \\ \cline{2-5} \cline{7-10} \cline{12-15} 
                         & NG@5            & NG@10           & HR@5            & HR@10           &           & NG@5            & NG@10           & HR@5            & HR@10           &  & NG@5            & NG@10           & HR@5            & HR@10           \\ \hline
Caser                    & 0.0161          & 0.0193          & 0.0224          & 0.0485          &           & 0.0122          & 0.0164          & 0.0187          & 0.0321          &  & 0.0042          & 0.0060          & 0.0069          & 0.0123          \\
GRU4Rec                  & 0.0248          & 0.0288          & 0.0342          & 0.0467          &           & 0.0169          & 0.0221          & 0.0261          & 0.0423          &  & 0.0060          & 0.0078          & 0.0094          & 0.0149          \\
SASRec                   & 0.0477          & 0.0535          & 0.0647          & 0.0824          &           & 0.0237          & 0.0290          & 0.0338          & 0.0502          &  & 0.0097          & 0.0123          & 0.0146          & 0.0226          \\
BIGRec                   & 0.0780          & 0.0945          & 0.1131          & 0.1631          &           & 0.0377          & 0.0434          & 0.0565          & 0.0742          &  & 0.0260          & 0.0333          & 0.0394          & 0.0612          \\
$D^3$                    & {\ul 0.0906}    & {\ul 0.1103}    & 0.1243          & 0.1826          &           & {\ul 0.0432}    & {\ul 0.0498}    & {\ul 0.0631}    & {\ul 0.0836}    &  & 0.0261          & 0.0329          & 0.0375          & 0.0585          \\ \hline
BIGRec+CFT               & 0.0855          & 0.1056          & {\ul 0.1309}    & {\ul 0.1925}    &           & 0.0398          & 0.0451          & 0.0608          & 0.0775          &  & {\ul 0.0292}    & {\ul 0.0359}    & \textbf{0.0449} & \textbf{0.0655} \\
$D^3$+CFT                & \textbf{0.0972} & \textbf{0.1203} & \textbf{0.1417} & \textbf{0.2116} & \textbf{} & \textbf{0.0453} & \textbf{0.0516} & \textbf{0.0674} & \textbf{0.0868} &  & \textbf{0.0298} & \textbf{0.0363} & {\ul 0.0435}    & {\ul 0.0635}    \\ \hline
\end{tabular}
}
\end{table*}



% \subsection{Analysis}
% \subsubsection{Ablation}
% \label{4.3.1}
% To investigate the impact of the parameters of CFT (\bm{$\alpha$} and \bm{$\beta$}) on recommendation performance across different datasets, we conducted ablation experiments here. The primary functions of these two parameters of are as follows: 1) $\alpha$ controls the weight of "difference" section, denoted by "Only Diff" 2) $\beta$ regulates the weight of tokens at different position, denoted by "Only Weighting". We deactivated each component individually to assess their impacts. The outcomes are collected in Table 2, leading us to the following conclusions:\\
% \begin{table*}[t]
% \centering
% \caption{Ablation Results for our method in terms of accuracy, "Baseline" denotes deactivating both components. "Only Diff" denotes activating  counterfactual reasoning. "Only Weighting" denotes activating the weighting mechanism}
% \begin{tabular}{clcccc}
% \hline
% {\color[HTML]{333333} Dataset}                                                                                  & \multicolumn{1}{c}{{\color[HTML]{333333} Metrics}} & {\color[HTML]{333333} \textbf{CFT}} & {\color[HTML]{333333} Only Diff} & {\color[HTML]{333333} Only Weighting} & {\color[HTML]{333333} Baseline} \\ \hline
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} NDCG@5}                      & {\color[HTML]{333333} \textbf{0.0855}}  & {\color[HTML]{333333} 0.0827}    & {\color[HTML]{333333} 0.0793}         & {\color[HTML]{333333} 0.0780}   \\
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} HR@5}                        & {\color[HTML]{333333} \textbf{0.1309}}  & {\color[HTML]{333333} 0.1264}    & {\color[HTML]{333333} 0.1184}         & {\color[HTML]{333333} 0.1131}   \\
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} NDCG@10}                     & {\color[HTML]{333333} \textbf{0.1056}}  & {\color[HTML]{333333} 0.1028}    & {\color[HTML]{333333} 0.0961}         & {\color[HTML]{333333} 0.0945}   \\
% \multirow{-4}{*}{{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}CDs\\ $\alpha$ = 0.025\\ $\beta$ = $\frac{1}{26}$ \end{tabular}}} & {\color[HTML]{333333} HR@10}                       & {\color[HTML]{333333} \textbf{0.1925}}  & {\color[HTML]{333333} 0.1884}    & {\color[HTML]{333333} 0.1702}         & {\color[HTML]{333333} 0.1632}   \\ \hline
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} NDCG@5}                      & {\color[HTML]{333333} \textbf{0.0398}}  & {\color[HTML]{333333} 0.0384}    & {\color[HTML]{333333} 0.0334}         & {\color[HTML]{333333} 0.0377}   \\
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} HR@5}                        & {\color[HTML]{333333} \textbf{0.0608}}  & {\color[HTML]{333333} 0.0578}    & {\color[HTML]{333333} 0.0492}         & {\color[HTML]{333333} 0.0565}   \\
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} NDCG@10}                     & {\color[HTML]{333333} \textbf{0.0451}}  & {\color[HTML]{333333} 0.0437}    & {\color[HTML]{333333} 0.0378}         & {\color[HTML]{333333} 0.0434}   \\
% \multirow{-4}{*}{{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}Games\\ $\alpha=0.02$\\ $\beta$=$\frac{1}{3}$\end{tabular}}}     & {\color[HTML]{333333} HR@10}                       & {\color[HTML]{333333} \textbf{0.0775}}  & {\color[HTML]{333333} 0.0742}    & {\color[HTML]{333333} 0.0628}         & {\color[HTML]{333333} 0.0742}   \\ \hline
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} NDCG@5}                      & {\color[HTML]{333333} \textbf{0.0292}}  & {\color[HTML]{333333} 0.0260}    & {\color[HTML]{333333} 0.0274}         & {\color[HTML]{333333} 0.0260}   \\
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} HR@5}                        & {\color[HTML]{333333} \textbf{0.0449}}  & {\color[HTML]{333333} 0.0393}    & {\color[HTML]{333333} 0.0411}         & {\color[HTML]{333333} 0.0394}   \\
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} NDCG@10}                     & {\color[HTML]{333333} \textbf{0.0359}}  & {\color[HTML]{333333} 0.0330}    & {\color[HTML]{333333} 0.0338}         & {\color[HTML]{333333} 0.0333}   \\
% \multirow{-4}{*}{{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}Books\\ $\alpha$=0.1\\ $\beta$ = $\frac{1}{1.2}$\end{tabular}}}    & {\color[HTML]{333333} HR@10}                       & {\color[HTML]{333333} \textbf{0.0655}}  & {\color[HTML]{333333} 0.0612}    & {\color[HTML]{333333} 0.0607}         & {\color[HTML]{333333} 0.0612}   \\ \hline
% \end{tabular}
% \end{table*}
% $\bullet$ Removing the counterfactual reasoning or the weighting mechanism will result in a decline in accuracy. These results underscore the significance of both designs in effectively tackling their specific challenges. \\
% $\bullet$ When utilizing counterfactual reasoning or the weighting mechanism to CFT, only one of the CFT designs is activated, the outcomes do not consistently exceed the baselines. Among the three datasets, only the CDs dataset surpassed the baselines with either approach. The Games and Books datasets exhibited marginal improvement or slight decline when applying a single method. This indicates that the integration of both methods can produce enhanced results. 

% \subsubsection{Parameters change}
% We have discussed the impact of various parameters on recommendation performance. Furthermore, we aim to investigate how changes in these parameters will affect the accuracy of recommendation. We conducted experiments on Books dataset. As shown in Figure \ref{}, we have the following findings: \\
% $\bullet$ With $\beta$ set to $\frac{1}{1.2}$, we achieved satisfactory recommendation performance at $\alpha$ values of 0.1 and 0.12. Significant declines in performance were observed at $\alpha$ values of 0.08 and 0.14. Therefore, we conclude that there exists an optimal range for $\alpha$ in the Books dataset.\\
% $\bullet$ When $\alpha$ is set to 0.1, we achieved the best predictive accuracy at $\beta$ values of $\frac{1}{1.2}$. We similarly propose that there exists an optimal range for $\beta$ in the dataset. 
% \subsubsection{Generalizability}
% To show the generalizability of our method, we conduct further experiments on more backbones and datasets. 


% \begin{table*}[t]
% \caption{Results on Steam dataset}
% \begin{tabular}{clcccc}
% \hline
% {\color[HTML]{333333} Dataset}                                                                                   & \multicolumn{1}{c}{{\color[HTML]{333333} Metrics}} & {\color[HTML]{333333} GRU4Rec} & {\color[HTML]{333333} SASRec} & {\color[HTML]{333333} BIGRec} & {\color[HTML]{333333} \textbf{CFT}}    \\ \hline
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} NDCG@5}             & {\color[HTML]{333333} 0.0250}  & {\color[HTML]{333333} 0.0282} & {\color[HTML]{333333} 0.0206} & {\color[HTML]{333333} \textbf{0.0338}} \\
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} HR@5}               & {\color[HTML]{333333} 0.0403}  & {\color[HTML]{333333} 0.0421} & {\color[HTML]{333333} 0.0337} & {\color[HTML]{333333} \textbf{0.0443}} \\
% {\color[HTML]{333333} }                                                                                          & {\color[HTML]{333333} NDCG@10}            & {\color[HTML]{333333} 0.0337}  & {\color[HTML]{333333} 0.0359} & {\color[HTML]{333333} 0.0250} & {\color[HTML]{333333} \textbf{0.0374}} \\
% \multirow{-4}{*}{{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}Steam\\ $\alpha$ = 0.55\\ $\beta$ = $\frac{1}{8}$ \end{tabular}}} & {\color[HTML]{333333} HR@10}              & {\color[HTML]{333333} \textbf{0.0676}}  & {\color[HTML]{333333} 0.0658} & {\color[HTML]{333333} 0.0479} & {\color[HTML]{333333} 0.0555} \\ \hline
% \end{tabular}
% \end{table*}

\subsection{Ablation Study (RQ2)}

\begin{table*}[t]
\caption{Results of the ablation study for our proposed CFT on three datasets with NDCG@$k$ (NG@$k$) and HR@$k$ as the metrics.}
\label{exp:abl}

\resizebox{0.98\textwidth}{!}{
\begin{tabular}{ccccccccccccccc}
\cline{1-10} \cline{12-15}
\multirow{2}{*}{Method} & \multicolumn{4}{c}{CDs}           &        & \multicolumn{4}{c}{Games}         &           & \multicolumn{4}{c}{Books}         \\ \cline{2-5} \cline{7-10} \cline{12-15} 
                        & NG@5   & NG@10  & HR@5   & HR@10  &        & NG@5   & NG@10  & HR@5   & HR@10  &           & NG@5   & NG@10  & HR@5   & HR@10  \\ \hline
BIGRec+CFT              & 0.0855 & 0.1056 & 0.1309 & 0.1925 & {\ul } & 0.0398 & 0.0451 & 0.0608 & 0.0775 & {\ul }    & 0.0292 & 0.0359 & 0.0449 & 0.0655 \\ \hline
- w/o Counterfactual                & 0.0793 & 0.0961 & 0.1184 & 0.1702 &        & 0.0334 & 0.0378 & 0.0492 & 0.0628 &           & 0.0274 & 0.0338 & 0.0411 & 0.0607 \\
- w/o Weighting         & 0.0827 & 0.1028 & 0.1264 & 0.1884 &        & 0.0384 & 0.0437 & 0.0578 & 0.0742 &           & 0.0260 & 0.0330 & 0.0393 & 0.0612 \\
- w/o Both              & 0.0780 & 0.0945 & 0.1131 & 0.1632 &        & 0.0377 & 0.0434 & 0.0565 & 0.0742 & \textbf{} & 0.0260 & 0.0333 & 0.0394 & 0.0612 \\ \hline
\end{tabular}
}
\end{table*}

\subsection{In-depth Analysis (RQ3)}

==> backup/not_use.tex <==

%%% with and without comparison on CDs Figure 4
\subfigure[ \textbf{CDs With History}]{ \includegraphics[width=0.23\textwidth]{figures/CDs_with_his.pdf}}
\subfigure[ \textbf{CDs Without History}]{ \includegraphics[width=0.23\textwidth]{figures/CDs_without_his.pdf}}
